Design Guidelines for High-Performance SCM Hierarchies

With emerging storage-class memory (SCM) nearing commercialization, there is evidence that it will deliver the much-anticipated high density and access latencies within only a few factors of DRAM. Nevertheless, the latency-sensitive nature of memory-resident services makes seamless integration of SCM in servers questionable. In this paper, we ask the question of how best to introduce SCM for such servers to improve overall performance/cost over existing DRAM-only architectures. We first show that even with the most optimistic latency projections for SCM, the higher memory access latency results in prohibitive performance degradation. However, we find that deployment of a modestly sized high-bandwidth 3D stacked DRAM cache makes the performance of an SCM-mostly memory system competitive. The high degree of spatial locality that memory-resident services exhibit not only simplifies the DRAM cache's design as page-based, but also enables the amortization of increased SCM access latencies and the mitigation of SCM's read/write latency disparity. We identify the set of memory hierarchy design parameters that plays a key role in the performance and cost of a memory system combining an SCM technology and a 3D stacked DRAM cache. We then introduce a methodology to drive provisioning for each of these design parameters under a target performance/cost goal. Finally, we use our methodology to derive concrete results for specific SCM technologies. With PCM as a case study, we show that a two bits/cell technology hits the performance/cost sweet spot, reducing the memory subsystem cost by 40% while keeping performance within 3% of the best performing DRAM-only system, whereas single-level and triple-level cell organizations are impractical for use as memory replacements.

==> Makefile <==
PAPER = ms
TEX = $(wildcard *.tex)
BIB = ref.bib
#../common/dblp.bib ../common/misc.bib ../common/morebibs.bib
FIGS = $(wildcard figures/*.pdf figures/*.png graphs/*.pdf graphs/*.png)

.PHONY: all distrib clean

$(PAPER).pdf: $(TEX) $(BIB) $(FIGS) acmart.cls
	echo $(FIGS)
	pdflatex $(PAPER)
	bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex $(PAPER)

bib: 
	./tools/bibcloud.py $(PAPER)
	bibtex $(PAPER)
spell:
	./tools/linearize.pl word $(PAPER).tex; open -a /Applications/Microsoft\ Word.app/ latex-all.tex

clean:
	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf 


==> abstract.tex <==
\begin{abstract}

\begin{comment}
\begin{itemize}
\item Replace DRAM with SCM for higher density / lower cost.
\item SCM latencies higher, especially for writes, resulting in severe bandwidth degradation -> challenging to replace DRAM.
\item Can get back lost bandwidth and match DDR bandwidth using SCM by larger data transfers, especially writebacks.
\item Servers will employ DRAM caches to cope with bandwidth wall. As also shown in prior work, modern server workloads exhibit significant spatial locality in modestly sized DRAM caches, a characteristic that can be leveraged to do bulk transfers between the DRAM cache and the backing SCM, for significant bandwidth improvements.
\item We further observe that the spatial density of writebacks is significantly larger than that of reads; hence the transfer granularity between the DRAM cache and the SCM cannot be fixed and needs to accommodate for this duality. 
\item We claim that DRAM caches are capable of bridging the performance gap between DRAM and SCM
thus paving the way for SCM integration in the memory hierarchy of future servers. However, maximizing their effectiveness requires smart techniques that accommodate for the disparity of SCM reads and writes. Our approach improves [...] 
\end{itemize}
\end{comment}

With emerging storage-class memory (SCM) nearing commercialization, there is evidence that it will deliver the much-anticipated high density and access latencies within only a few factors of DRAM. Nevertheless, the latency-sensitive nature of in-memory services makes seamless integration of SCM in servers questionable. In this paper, we ask the question of how best to introduce SCM for such servers to help improve overall performance per cost over existing DRAM-only architectures. We first show that even with the best latency projections for SCM, the higher memory access latency results in prohibitive performance degradation. However, we find that deploying a modestly sized high-bandwidth stacked DRAM cache makes SCM-based memory competitive. The high degree of spatial locality in-memory services exhibit not only simplifies the DRAM cache's design as page-based, but also enables the amortization of increased SCM access latencies and mitigation of SCM's read/write latency disparity. We finally perform a case study with PCM, and show that a 2 bits/cell technology hits the performance/cost sweet spot, reducing the memory subsystem cost by 40\% while keeping performance within 5\% of the best performing DRAM-only system, whereas single-level and triple-level cell organizations are impractical for use as memory replacements. 
%Our results indicate that both multi-level cell PCM and ReRAM lifetime can be improved by an order of magnitude, by sacrificing the excessive write speed, while keeping overall performance within 7\% of the DRAM-based system.

%4$\times$-64$\times$


%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
With emerging storage-class memory (SCM) nearing commercialization, there is evidence
that it will deliver the much-anticipated high density and access latencies within
only a few factors over DRAM. SCM will be most disruptive if it can prove capable to
replace DRAM as main memory. Such replacement can greatly reduce the DRAM-dominated cost
of high-memory server systems.

In this work, we demonstrate the potential of SCM as a main memory replacement for DRAM-based main memory. While a simple replacement results in severe performance degradation, we show that a simple 3D stacked cache design, organized in multi-KB cache blocks, can bridge that performance gap even for memories with 100-1000s of ns access latency, by leveraging abundant spatial locality of server applications. The two-level memory hierarchy proposed relaxes latency/bandwidth requirements for backing memory level, providing SCM designers with sufficient performance headroom to enhance SCM's non-performance characteristics, such as cost/bit and endurance, by sacrificing excessive SCM speed. To help SCM device experts, we devise a performance/cost model that provides design directions for upcoming SCM technologies. We show the utility of the model by doing case studies with Phase-Change Memory (PCM) and Resistive RAM (ReRAM) memories. We show that PCM memory that stores 2 bits/cell hits the performance/cost sweet spot, reducing the memory subsystem cost by 30\% while keeping performance within 5\% of the best performing DRAM-only system, whereas its single-level and triple-level cell organizations are not practical. For ReRAM, we show that its endurance can be improved by 4-64$\times$, by sacrificing its excessive write speed, while keeping overall performance within 7\% of the DRAM-based system. 

%%%%%%%%%%

In this work, we investigate the potential of SCM as a replacement for DRAM-based main
memory. While a simple replacement results in severe performance degradation, we show
that a careful design of the memory hierarchy can bridge that performance gap. We 
study the access patterns of modern server workloads and find that (i) there is abundant
spatial locality, and (ii) writes are significantly more spatially correlated than
reads, a characteristic that matches the read/write latency disparity of SCM.
We leverage these observations to amortize the high access latency of SCM and 
alleviate its bandwidth limitations. We design Janus, an SCM-aware DRAM cache that 
accommodates for the duality of SCM reads and writes by moving data at different
granularities, and show that a server with an SCM-based memory and a modestly sized 
Janus cache approaches the performance of a DRAM-only system within 3\% and 8\% %17\% 
with high performance and high density SCM-based memory, respectively. 
\end{comment}

\end{abstract}

==> floats/float-3scm-perf.tex <==
\begin{figure}[t]
\centering
        \includegraphics[width=0.95\columnwidth]{figures/3perf}
\caption{System performance with different SCM solutions with 2KB block size, normalized to DRAM-based system.}
\label{fig:3scm_perf}
%\vspace*{-9pt}
\end{figure}


==> floats/float-cost-perf.tex <==
\begin{figure}[t]
\centering
        \includegraphics[width=0.95\columnwidth]{figures/cost_perf}
\caption{Cost/performance design space for DRAM and SCM configurations.}
\label{fig:cost_study}
%\vspace*{-9pt}
\end{figure}

==> floats/float-dimm-organization.tex <==
\begin{figure}[t]
        \centering
        \includegraphics[width=0.8\columnwidth]{figures/dram-internals}
        \caption{DIMM organization.}
        \label{fig:dimm_organization}
       % \vspace*{-9pt}
\end{figure}

==> floats/float-janus-design.tex <==
\begin{figure*}[t]
        \centering
        \includegraphics[width=1.8\columnwidth]{figures/janus_organization}
        \caption{DRAM page cache organization.}
        \label{fig:janus}
       % \vspace*{-9pt}
\end{figure*}


==> floats/float-lat-sensi.tex <==
\begin{figure*}[t]
\centering
\subfloat[Sensitivity to symmetric SCM latencies (tRCD=tWR).]{
       % \hspace{6pt}
        \includegraphics[width=0.95\columnwidth]{figures/symm_sensi}
        \label{fig:symm_sensi}}
\subfloat[Sensitivity to read/write disparity (tRCD=500ns).] {
        \includegraphics[width=0.95\columnwidth]{figures/disparity_sensi}
        \label{fig:disparity_sensi}}
\caption{SCM-based system sensitivity to SCM latencies and read/write disparity (GEOMEANs).}
\label{fig:sensitivity}
%\vspace*{-9pt}
\end{figure*}

==> floats/float-pcm-metrics.tex <==
\begin{figure}[t]
\centering
       % \hspace{6pt}
        \includegraphics[width=\columnwidth]{figures/pcm_metrics}
\caption{Performance and cost metrics of various DRAM- and PCM-based hierarchies.}
\label{fig:pcm_metrics}
%\vspace*{-9pt}
\end{figure}


==> floats/float-perf.tex <==
\begin{figure}[t]
\centering
        \includegraphics[width=0.95\columnwidth]{figures/tlc_perf}
\caption{\textit{Dense} SCM-based systems performance, normalized to DRAM-based system.}
\label{fig:perf_study}
%\vspace*{-9pt}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure*}[t]
\centering
\subfloat[High performance SCM.]{
       % \hspace{6pt}
        \includegraphics[width=0.95\columnwidth,height=0.47\columnwidth]{figures/fast_perf}
        \label{fig:fast_perf}}
\subfloat[High density SCM.] {
        \includegraphics[width=0.95\columnwidth,height=0.47\columnwidth]{figures/dense_perf}
        \label{fig:dense_perf}}
\caption{SCM-based systems performance, normalized to DRAM-based baseline system.}
\label{fig:perf_study}
%\vspace*{-9pt}
\end{figure*}
\end{comment}

==> floats/float-traffic.tex <==
\begin{figure*}[t]
\centering
\subfloat[SCM row activations.]{
       % \hspace{6pt}
        \includegraphics[width=0.65\columnwidth]{figures/act_traffic}
        \label{fig:act_traffic}}
\subfloat[Read traffic.]{
       % \hspace{6pt}
        \includegraphics[width=0.65\columnwidth]{figures/read_traffic}
        \label{fig:read_traffic}}
\subfloat[Write traffic.] {
        \includegraphics[width=0.65\columnwidth]{figures/write_traffic}
        \label{fig:write_traffic}}
\caption{Characteristics of the traffic to SCM, normalized to a system with a regular DRAM cache with 1KB blocks.}
\label{fig:traffic_study}
%\vspace*{-9pt}
\end{figure*}


==> obsolete/BACKUP_INTROS.tex <==

\begin{comment}

\noindent\rule[0.5ex]{\linewidth}{1pt}

\textbf{Paper flow:}
\begin{enumerate}
    \item Server workloads are data-driven. Memory is first-class system component and major cost contributor.
    \item SCM soon commercialized, appealing alternative to DRAM because of high density $\rightarrow$ higher capacity / lower cost. Access latency not dramatically higher than DRAM (within few factors). Can we deal with reduced performance and read/write disparity of SCM and use it as
    DRAM replacement?
    \item Direct replacement of DRAM w/ SCM $\rightarrow$ \textbf{NO!} Timing results to illustrate dramatic degradation.
    \item Prior work has shown that modestly sized DRAM caches can capture a lot of locality of server applications. Can we use a DRAM cache to mitigate performance degradation of using SCM as main memory?
    \item Workloads analysis: separate temporal from spatial locality. Bullshit about reasonable cache size being $\sim$3\%.
    \item Insight: point out that abundant spatial locality, more spatial locality for writes, fits greatly SCM read/write disparity. Spatial locality
    enables possibility of bulk transfers; show how bulk transfers can amortize high SCM access latency.
    \item Qualitatively reason about cache organizations. Block-based cache cannot capture spatial locality, kills SCM bandwidth with fine-grained
    accesses. Make case for cache with dual transfer size for reads and writes: Large units of transfer (optimized for writes) mitigate bandwidth degradation because of slow writes, but cause overfetch for clean regions. Small units of transfer (optimized for reads) preserve read bandwidth, but result in small writes that hurt the effective BW of SCM. \textbf{Need duality in block size: smaller for reads, larger for writebacks.}
    \item Evaluated systems (TIMING):
    \begin{itemize}
        \item Cache w/ 64B blocks $\rightarrow$ improves over SCM-only, but only captures temporal locality
        \item Cache w/ small pages $\rightarrow$ small writes kill BW
        \item Cache w/ large pages $\rightarrow$ overfetch
        \item Cache w/ dual transfers (Sector cache?) $\rightarrow$ nails it (hopefully doesn't outperform DRAM baseline :D)
        %\item Solution: pick block size tailored to reads, create larger virtual regions for writebacks using variant of Virtual Write Queue.
    \end{itemize}
\end{enumerate}
\noindent\rule[0.5ex]{\linewidth}{1pt}
\end{comment}

\begin{comment}
\noindent\rule[0.5ex]{\linewidth}{1pt}
Intro:
\begin{itemize}
\item Motivate for replacing DRAM with SCM. Data intensive services, memory centric computing, DRAM dominates price of server.
\item SCM is promising alternative: much denser (order of magnitude), not dramatically slower than DRAM.
\item Show performance graph: can't just replace DRAM with SCM.
\item Server workloads exhibit high locality that DRAM caches can capture. Especially abundant spatial locality can enable
large transfers to amortize high latency of SCM accesses, boosting the bandwidth. Our study shows that writes are significantly
more spatial than reads, allowing larger batches, which is a great fit for the read/write disparity of SCM.
\item We show that, while a modestly sized DRAM cache can dramatically boost the performance of a memory hierarchy with SCM
as main memory, simple organizations are suboptimal. Small blocks result in low bandwidth from SCM, large blocks overfetch. Need duality.
\end{itemize}
\noindent\rule[0.5ex]{\linewidth}{1pt}


\dmitrii{New motivation: (1) memory expansion, (2) cost/bit, (3) static power reduction}

\dmitrii{add subsection on SCM DIMM design with wide row buffers decoupled from S/A, citing Yuan}

\dmitrii{add a section on SLC, MLC, TLC perf \& cost model}
\end{comment}
%========================================================================================================================================
%========================================================================================================================================
%========================================================================================================================================

\begin{comment}
\noindent\rule[0.5ex]{\linewidth}{1pt}
Story
\begin{itemize}
    \item Conventional (DRAM-based) memory can account for up to 50\% of the server cost. Emerging (SCM-based) memories are expected to reduce the cost coming at much lower cost per bit and moderate endurance, but a straightforward replacement of DRAM is not possible even for performance-optimized SCMs due to large performance differences, while density-optimized SCMs are much slower.
    \item Prior work on server workload characterization has shown that even though there is little data locality in even the largest on-chip caches, significant reuse can be captured by DRAM caches. Driven by this observation, we show that a properly designed DRAM cache enables the replacement of DRAM-based memory with slower but cheaper SCM of certain characteristics, without significant performance degradation. 
    \item In this work, we show that there is abundant spatial locality in cloud workloads at the memory level, and how it can be exploited to bridge the SCM-DRAM performance gap.
    \item SCM technologies are very diverse in terms of their latency, bandwidth, and read/write performance disparity characteristics as a function of the used cell, reflecting into the cost/bit as well. The challenge lies in picking the right configuration that minimizes the memory subsystem's total cost (DRAM cache + SCM memory), while meeting the performance goals.
    \item We devise DESPACITO, a performance and cost model, to hash out the design space for memory hierarchies with SCM-based memory. Using DESPACITO's performance model, we identify all memory subsystem configurations (DRAM cache + SCM characteristics) that are viable options as replacements of DRAM-only solutions. We then use its cost model to identify the configurations with the best performance/cost, and show that DRAM-only memory hierarchies can be replaced by similarly performing SCM + DRAM cache configurations that are up to XXXX$\times$ cheaper. 
    \item DESPACITO also provides design directions for upcoming SCM technologies. SCM technology and device experts can leverage the model to identify the combination of parameters (latency, bandwidth, and read/write disparity) that make a given SCM device a fitting candidate for a server's memory hierarchy.
    \item We demonstrate the utility of DESPACITO with two case studies, and show that:
    \begin{enumerate}
    \item PCM read latency and disparity can be traded off for higher density (thus, cost reduction). We show that storing 2 bits/PCM cell is the sweet spot, as 1 bit/cell does not offset the cost of the DRAM cache, and storing 3 bits/cell leads to unacceptable performance degradation.
    \item A ReRAM-based memory can tolerate $N\times$ write latency degradation for a $N^{1-3}\times$ increase endurance, without sacrificing performance. We show that given 200ns/200ns original read/write latency, endurance can be improved by 4-64$\times$. 
    \end{enumerate}

\end{itemize}

\noindent\rule[0.5ex]{\linewidth}{1pt}
Contributions:
\begin{itemize}
    \item Showed that SCM can replace DRAM
    \item SCM requires a cache in front
    \item Cache has to be highly parallel inside, and organized in blocks sized according to data locality and SCM row buffer size.
    \item Devised a design exploration framework for SCM, based on three architectural/memtech parameters, that can be used by SCM and CPU architects to build cheaper yet high performance servers.
    \item Demonstrated the use of the framework for case studies with examples of PCM and ReRAM technologies.
\end{itemize}
\noindent\rule[0.5ex]{\linewidth}{1pt}


\dmitrii{Intro has to be rewritten according to the story above}

The booming popularity of online services raises the demands for modern servers. 
Memory takes center stage, as services are becoming increasingly more data-intensive
and each user request requires massive dataset traversals.
As a consequence, keeping data memory-resident
has become common practice, a trend that results in server systems with increasing DRAM capacity
that accounts
for a major fraction of the infrastructure's cost\footnote{DRAM can account for more than 50\% of a high-memory server's cost.
To illustrate, the cost of the processor and DRAM in a 2-socket server with a mid-range Xeon (E5-2660) and 512GB of memory
is about \$3000 and \$6500, respectively.}. \dmitrii{The demand for high memory density is 
growing fast, for example, Amazon EC2 plans to deploy server instances with up to 16TB of 
memory \cite{amazon:ec2}. As DRAM scalability has been lagging behind, memory vendors 
have started exploring alternative technologies.}
Storage-class memory (SCM) technologies emerge as appealing candidates to replace DRAM, 
and going to be available soon as commercial products, such as Intel and Micron's 3D XPoint~\cite{intel:3dxpoint}.
With an access latency that is only a few factors higher than DRAM and an order of magnitude higher
density---which can result in commensurate cuts in memory cost---SCM is a main memory alternative
worth investigating. As first commercial products are expected to be optimized for high performance (storing a single bit per cell), and similar or slightly less cost/bit \cite{computerworld:3dxpoint,zhou:hnvm,wd:reram} as DRAM, we envision that further generations are going to focus on delivering more density, as the main economical advantage of SCM. SCM's density is expected to grow by putting more bits per SCM cell \cite{stanisavljevic:demonstration}, which may provide almost linear decrease of cost/bit, or 3D stacking of multiple SCM layers \cite{intel:3dxpoint,wd:reram}. Unfortunately, both ways are going to degrade read, and especially write access latencies futher. Thus, server architects have to adopt their designs for 10-100$\times$ higher memory access latencies to leverage SCM's high capacity for memory-intensive workloads that are ubiquitous in modern datacenters \cite{ferdman:clearing}.

\dmitrii{TBD: can cite \cite{hirofuchi:raminate} for DRAM energy consumption reduction with LPDDR kinda ifaces,
}

Unfortunately, simply replacing DRAM with SCM can significantly hurt performance. 
Fig.~\ref{fig:scm_vs_dram} shows the relative performance of a server using SCM as main 
memory---with $4\times$/$10\times$ slower reads/writes than DRAM, respectively---
as compared to conventional DRAM, on a range of modern server workloads.
Across five different evaluated workloads, replacing DRAM main memory with
SCM results in a 40\% performance drop on average, with some workloads' throughput
dropping by half. In general, the higher the bandwidth requirements and write intensity of
the workload, the higher performance degradation it suffers.
Clearly, regardless of the potential cost benefits from deploying SCM-based memory instead of
DRAM, such a performance drop is unacceptable.

In this work, we investigate memory hierarchy design options that will mitigate
this performance degradation, making SCM main memory a viable choice for servers.
We study a set of modern server workloads and find access patterns that exhibit significant
locality that can be captured in a modestly sized DRAM cache, corroborating findings in prior work
\cite{jevdjic:die-stacked, volos:fat, volos:bump}. More importantly, a large fraction of
this locality is spatial, a characteristic that can be leveraged to amortize the high latency of SCM access:
by turning fine-grained accesses to bulk, it is possible to approach required memory bandwidth, as sequential read and especially write bandwidth of emerging memories is projected to be around an order of magnitude higher than for random accesses \cite{suzuki:nonvolatile}.
In addition, we find that writes in server workloads are significantly more spatial than reads.
The duality in spatial density between reads and writes greatly fits the read/write disparity of SCM, as
it enables orchestration of even larger accesses for writes, required to amortize their higher latency.

Building on our observations, we investigate memory hierarchy designs that can enable replacement of DRAM-based memory
with SCM, with minimal loss in performance\dmitrii{ without increasing the overall cost of 
the memory subsystem}. We show that this goal is achievable by deploying a modestly sized DRAM cache with large blocks sized to match 
the spatial locality of server workloads and amortize SCM's high access latency. \dmitrii{just advocate for a page cache?} 
However, the cache's organization has a significant impact on
performance: Sizing the cache block to best fit the spatial locality of either reads or writes
is suboptimal. The former results in smaller writes than possible, thus reducing SCM's effective bandwidth. The latter
results in severe data overfetch and hence bandwidth misuse, as the reads exhibit much lower spatial locality than writes.
We therefore propose an SCM-aware DRAM cache organization for servers that is tailored to the read/write disparity trait
of SCM technologies, the Janus cache\footnote{Janus is the Roman god with two faces, looking into future and past, 
as data reads and writes are for the processor}. Janus exhibits a \textit{dual} nature, by treating reads and writebacks differently.
While organized in cache blocks whose size is tailored to the spatial locality of reads, it groups multiple blocks into larger
virtual regions, which are evicted in bulk, sized to match the spatial locality of writes.
%\dmitrii{Describe the design options. Consider 2 SCM types.}
We make the following contributions:

\begin{itemize}
    \item We observe that the high access latency of SCM can be amortized with larger transfers, enabling SCM to deliver
    bandwidth comparable to DRAM.
    \item We analyze a number of representative modern server workloads and 
    illustrate that they exhibit high spatial locality,
    which can be exploited to make bulk accesses to SCM and thus extract high bandwidth. 
    \item We further make the novel observation that read/write disparity in emerging memory 
    does not play an essential role, despite the fact that writes exhibit 
    significantly higher spatial locality than reads.\dmitrii{revisit}
    \item We show that a high-bandwidth DRAM cache with a size that only accounts for a minuscule fraction of its
    backing memory can successfully mitigate the performance shortcomings of SCM.
    \item We demonstrate that a simple page cache, tailored to the characteristics of the target workloads, 
    hits system cost/performance sweet spot for a wide range of SCM characteristics, providing performance within \dmitrii{92-99\% of the DRAM-based system} 
    at 20-50\% lower memory subsystem cost, without adding design complexity.

%\begin{comment}
    \item We analyze a number of representative modern server workloads and illustrate that they exhibit high spatial locality,
    which can be exploited to make bulk accesses to SCM and thus extract high bandwidth. We further make the novel observation that
    writes exhibit significantly higher spatial locality than reads; this is especially fortunate for systems with SCM-based memory, as it allows for
    even larger write batches, capable of amortizing SCM's high write latency.
    \item We show that a DRAM cache with a size that only accounts for a minuscule fraction of its
    backing memory can successfully mitigate the performance shortcomings of SCM.
    However, the cache's design has to be tailored to the characteristics of the target workloads and the read/write disparity
    idiosyncrasy of SCM. We propose the Janus cache design, an SCM-aware DRAM cache,
    which handles reads and writebacks in different granularities to maximize SCM's useful bandwidth utilization.
    \item We demonstrate that a high performance SCM-based system can achieve performance within 3\% of a DRAM-based system,
    by making maximum use of abundant spatial locality captured by a DRAM cache at the right granularity.
    Also, we show that the proposed cache design enables performance within 8\% %17\% 
    of the DRAM-based system
    for a high density SCM-based system, outperforming the naive page cache designs by 11\%%10\%
    .
%\end{comment}
\end{itemize}

\dmitrii{intro to be written}

%\input{floats/float-scm-vs-dram}

The rest of the paper is organized as follows: 
\S\ref{sec:background} provides a background on emerging SCM technologies, and disputes the possibility of a drop-in DRAM replacement, advocating for increasing data transfer granularity to amortize high SCM latency.
%and illustrates the opportunity of latency amortization through bulk accesses.
We analyze the access patterns of server workloads in \S\ref{sec:workloads}
and identify a match between their spatial locality and the SCM row buffer sizes required to accommodate
for high access latency, and demonstrate that a page-based stacked DRAM cache design can bridge the performance gap.
As placing a stacked DRAM cache increases overall system cost, we use main SCM parameters to draw the SCM hierarchy design in  \S\ref{sec:approaches}.
We outline our methodology in \S\ref{sec:method}. We quantify the SCM hierarchy design space in \S\ref{sec:eval}, and perform a case study with phase-change memory to determine its performance and cost implications for in-memory services. We analyze our work implications for the software that takes advantage of SCM non-volatility in \S\ref{sec:disc}.
Finally, we discuss related work in \S\ref{sec:related} and conclude in \S\ref{sec:conclusion}.

\end{comment}

%========================================================================================================================================
%========================================================================================================================================
%========================================================================================================================================


\begin{comment}
\noindent\rule[0.5ex]{\linewidth}{1pt}

\textbf{Motivation.} 
The datacenter market shows an exponential growth over the years. To meet tight Quality-of-Service guarantees, the applications tend to store their datasets in the main memory of a number of servers, making memory a valuable, often scarce, resource and significant fraction of server TCO. With DRAM being the dominating memory technology, technological scaling of memory cells struggles to keep up with rapidly growing applications datasets. Despite significant investments by main DRAM vendors like Micron and Samsung, DRAM's density lags behind the capacity demands of the applications, giving a way for new emerging memory alternatives, usually referred as storage-class memory~(SCM) technologies, like phase-change memory~(PCM), resistive RAM~(ReRAM), or spin-transfer torque memory (STTRAM) that promise much higher density at much lower cost per bit.


\textbf{Problem.} Datacenter applications pose both low latency and high bandwidth requirements for the in-memory storage. In particular, bandwidth demands of modern servers are projected up to tens and hundreds of Gb/s, sufficiently exceeding the throughput of commodity, and even high-end, DRAM DIMMs. 
Performance characteristics (writes/reads disparity) of SCM prohibit direct replacement due to lack of available bandwidth, and high access latency. Related work focuses on increasing available bandwidth by boosting intra-rank parallelism of SCM DIMMs, apply writes filtering techniques using a DRAM . However, even achieving maximum IRLP cannot provide enough BW to supply state-of-the-art CPUs. One of the solutions to the Bandwidth Wall problem, described above, is placing a large DRAM cache (e.g., Micron's HMC, or Hynix HBM) in front of the main memory DIMMs. However, even with >90\% DRAM cache hit ratio, the main memory traffic may be challenging to serve even from fast DRAM-based DIMMs. The disparity of read and write PCM latencies degrades available PCM bandwidth even further forcing system designers to use many-rank heterogeneous systems (e.g., 32-rank PCM-based memory~\cite{ham:disintegrated}) that negates the cost savings of using a cheaper memory technology.

\textbf{Insights.} In this paper, we show that abundant locality captured by a DRAM cache of a sufficient size enables sufficient throughput from dense PCM-based memory DIMMs, helping significantly reduce the price of a commodity server. Corroborating a similar insight for DRAM devices~\cite{stuecheli:vwq}, we show that increasing burst length per access may unleash high memory throughput out of relatively slow PCM devices, just by leveraging row buffer locality of a conventional DIMM design. 

\textbf{Design.} To get a optimal burst length of the main memory accesses, the DRAM cache has to be organized in a way that it accounts for high latencies of read and especially write accesses to PCM-based devices. Ina  presence of a severe 4-12x write/read latency disparity of PCM, this insight motivates for using different effective burst lengths for read and write accesses, that implies bimodal management of read-only and dirty cache blocks in a DRAM cache. 

\textbf{Contributions.}
\begin{itemize}
	\item We show that scarce bandwidth of in-memory storage prohibits direct replacement of DRAM with slower, though much cheaper, PCM technology.
	\item We demonstrate that increasing burst length of memory accesses allows to significantly improve PCM-based memory throughput and queueing delays.
	\item We propose a DRAM cache design that enables efficient PCM accesses of bimodal granularity for read and writeback requests, only by leveraging abundant spatial locality of datacenter workloads, by minor modification of a conventional page-based DRAM cache.
	\item This is the first paper, to the best of our knowledge, that shows that PCM-based server can deliver performance within ?\% of a DRAM-based system for extremely bandwidth- and latency-constrained datacenter workloads.
\end{itemize}

\end{comment}

==> obsolete/OLD_S3_FRAGMENTS.tex <==

\begin{comment}
\noindent\rule[0.5ex]{\linewidth}{1pt}
Layout:
\begin{itemize}
    \item Server workloads have high BW requirements, producing 0.4-1.2GB/s \cite{jevdjic:die-stacked} per core, that boils down to high memory BW utilization, as the logic continues to scale faster than he number of pins.
    \item Prior work showed that die-stacked DRAM caches can significantly improve performance of DRAM-based system, as they have much higher internal parallelism, hence, much lower queuing delays. 
    \item Although prior work advocated to cache 10-15\% of the dataset (give examples), it's impractical due to expected order of magnitude increase of memory density brought by SCM.
    \item Stacked caches are expensive (7x more expensive than planar DRAM for 16-layer integration), so their capacity has to be small. Only 3-6\% can be practical provided that their cost can be offset by making the main memory cheaper.
    \item We use trace simulation to to determine cache size and block size to capture necessary data locality.
    \item We sweep cache size from 0.1\% to 12\% of the whole dataset, and show that for miss ratio can be brought down to below 5\% leveraging abundant spatial locality.
    \item To understand bulk accesses efficiency we study data region density for reads and writes. We point out that writeback locality is high, that should result in efficient bulk writebacks w/o significantly increasing writeback traffic, whereas read traffic granularity is much lower and requires careful use to avoid fetching useless data.
\end{itemize}
\noindent\rule[0.5ex]{\linewidth}{1pt}


\noindent\rule[0.5ex]{\linewidth}{1pt}

\dmitrii{need to add examples of dense dirty regions: logs, analytics' output to column-oriented stores, client connection's buffers, big KV objects, persistence-related writes \cite{zhao:firm}}

\begin{itemize}
    \item briefly talk about server workloads, and why DRAM caches are needed for BW. DRAM caches can cover for the latency.
    \item For a range of server workloads, show how density of clean and dirty regions changes with cache size.
    \item Establish that reads dominate the accesses and writebacks are much denser. Give qualitative reasons why. \dmitrii{in future, we may want to outline a special case of singleton writes that seems to be a common case as well, e.g., hashtable update}
    \item Need to balance memory subsystem to optimize for both frequent accesses (reads) and expensive accesses (writebacks). Tradeoff is new, because of RD/RW disparity in SCM.
\end{itemize}

\noindent\rule[0.5ex]{\linewidth}{1pt}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% WRITE HERE 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\rule[0.5ex]{\linewidth}{1pt}
Mark Layout:
\begin{itemize}
    \item We study the applications from CS and show that performance suffers greatly when attempting to directly drop-in SCM DIMMs.
    \item Degradation occurs because the applications do not make use of the spatial locality in each row buffer, directly exposing the activation and restoration latencies.
    \item Cite prior work saying that there is actually abundant spatial locality but it is not possible to be captured at the row buffer of the memory. cite bump.
    \item But we get much less BW with typical row buffers, then we choose a high-BW cache, which has to be 3D DRAM. 
    %\item The cache must be 3d DRAM, not planar, due to raw bandwidth requirements (shown previously).
    \item Due to the high cost of 3d DRAM, we need to find the minimal size that allows us to capture the application's working set (classical knee of curve analysis).
    \item We show the 3\% graphs and explain.
    \item This 3d cache needs to be architected as a page cache due to low temporal locality in applications. Using a block-based cache means that a large fraction of SCM accesses will incur the high latencies of opening a new SCM row.
    \item Applications have sufficient \emph{spatial} density inside each cached page in order to amortize the activation costs of the SCM memory (as shown in previous section).
    \item Conclude, we show that a Pg based 3d D\$ enables us to replace DRAM with SCM as the main memory, based on the fundamental observation that we need to amortize SCM activations. Commment on figure showing block size approaching page size.
    \item Next section shows how to choose the correct SCM organization to reduce the cost of the 3d D\$.
\end{itemize}
\noindent\rule[0.5ex]{\linewidth}{1pt}
\end{comment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

The other applications exhibit high region densities for typical SCM row buffer sizes, which motivates us to design our DRAM cache with the following guidelines in mind:
\begin{enumerate}
    \item Capacity should be approximately 3\% of the backing SCM.
    \item The cache should hold pages of the maximum size possible to match the backing SCM's row buffer. We argue for the use of 2KB pages.\javier{What's the size of the SCM row buffer?}
    \item Even if the SCM supports larger row buffers, do not use larger pages in the DRAM cache due to bandwidth overfetching.\javier{The last two bullets are contradictory. }
\end{enumerate}










As we have illustrated in Fig.~\ref{fig:scm_vs_dram}, replacing a server's DRAM with SCM results in severe performance degradation, because of SCM's high latency and low bandwidth. To bridge the performance gap with conventional DRAM, researchers proposed adding a DRAM cache. The DRAM cache design is the essential part of the SCM-based hierarchy, as the cache has to efficiently hide high delays of the SCM memory. To achieve this challenging goal, we analyze the characteristics, such as memory traffic and data locality, of a number of representative server workloads from CloudSuite~\cite{ferdman:clearing}.
%researchers proposed heterogeneous integration of both SCM and DRAM in the same system, while using DRAM as a software- \cite{hirofuchi:raminate} or hardware-managed \cite{qureshi:scalable} cache.

Prior work \cite{jevdjic:die-stacked,volos:fat} demonstrated that server workloads produce a large amount of memory traffic, setting up the "memory bandwidth wall" for the DRAM cache to overcome. High utilization of conventional DDR channels and limited parallelism inside conventional DIMMs causes high queuing delays that leads to high average memory access latency, and poor overall performance. To mitigate the bandwidth wall, both researchers and industry are actively looking into high bandwidth 3D stacked DRAM technology, such as Micron's Hybrid Memory Cube~(HMC) and Hynix' High Bandwidth Memory (HBM) \cite{micron:hmc,amd:hbm}. Such solutions employ a fast wide memory interface, and use 100s of independent DRAM banks. According to our results, using a high-bandwidth DRAM cache in front of conventional DRAM DIMMs increases server applications performance up to 2.3$\times$, as compared to a system that uses only planar DRAM, corroborating prior work \cite{jevdjic:die-stacked,volos:fat}. However, 3D stacked DRAM caches are expensive, and increase system integration complexity, slowing down its penetration to server market. We expect emerging highly dense SCM solutions to significantly reduce the cost of the memory subsystem, offsetting the cost of adding an expensive 3D stacked DRAM cache to the memory hierarchy. However, this would be possible provided that the overall system cost is reduced while overall system performance still satisfies QoS guarantees.

Prior work advocating for DRAM caches for servers
has indicated that server workloads exhibit significant locality that can be captured by reasonably sized caches to
boost performance \cite{jevdjic:die-stacked, volos:fat}. In the case of DRAM caches for SCM-based memory, there are three main
differentiating factors in terms of design limitations and performance impact: 
\begin{enumerate}
\item [(i)] the relative capacity of the DRAM cache as compared to its backing main memory is much more limited, as SCM can be an order of magnitude denser than DRAM \cite{wd:reram},
\item [(ii)] the cache hit ratio can dramatically improve the access latency, as it eschews a significantly higher SCM access latency.
%, and 
%\item [(iii)] special care has to be taken to cope with read/write disparity, a characteristic that is absent from DRAM.
\end{enumerate}

Putting things into perspective regarding factor (i), the size of a DRAM cache backing the planar DRAM on a single 
memory channel today can reasonably measure up to 64GB \cite{opencompute} capacity (assuming an 8GB HMC-like cache and 64GB of
DRAM per channel). With an expected density increase of about an order of magnitude when moving from DRAM to SCM (i.e., from
64 to 640GB), 
this size fraction will drastically drop to a 3-6\% range, even if we assume a doubling or quadrupling of the DRAM cache's
density (i.e., from 8 to 16 or 32GB). 
While prior work \cite{volos:fat} has advocated for DRAM caches in the 10-15\% capacity as an efficiency
sweet spot for servers with DRAM-based memory, such capacity ranges are clearly out of scope for SCM-based systems, as such cache could nearly double the cost of the memory subsystem \cite{dong:fabrication}.

To investigate whether reasonably---in the context of SCM---sized DRAM caches can leverage the locality of server workloads
to cover for the loss in performance because of the slower memory, we study a set of representative server applications from
CloudSuite \cite{ferdman:clearing}. We set up our experiments to investigate whether the expected spatial locality is enough to achieve the target amortization illustrated in \S\ref{sec:latency_amortization}.

\noindent\textbf{Data locality analysis.} 
We employ trace simulation and sweep through cache sizes, in the capacity range that is reasonable for a 
DRAM cache backing SCM main memory. We model a fully-associative cache, organized in blocks of a size in 
range from 64 to 4096 bytes. For brevity, we show the results only for \dmitrii{256, 1024 and 4096} bytes, 
as they correspond to typical SCM row buffer sizes \cite{suzuki:nonvolatile} that physically constrain 
available SCM bandwidth. Fig.~\ref{fig:locality} plots the miss ratio of such a cache as a function of the 
cache's capacity, which is expressed as a fraction of the dataset size; details on the methodology are 
provided in \S\ref{sec:method}. The workloads exhibit high data locality, although locality of different 
workloads varies. Data Analytics is insensitive to the cache size, and exhibits very high locality even for 
small caches. Web Search behavior demonstrates a dramatic step function in miss ration when growing the 
cache from 3 to 6\%, indicating that its primary working set is a small fraction of its dataset. Finally, 
the rest of the workloads exhibit a smoother reduction in miss ratio as the cache size grows. In all cases, 
a cache in the reasonable 3-6\% capacity range is capable of capturing a significant amount of the 
workloads' locality. Fig.~\ref{fig:1KB_locality} shows that organizing the cache of the same size in 1KB 
rather than 256B blocks dramatically shrinks the miss ratio of all workloads to sub-5\% ranges even for 
modest caches sizes (>2\%). Furthermore, there is no perceivable benefit from growing the cache size beyond 
a 2\% capacity: the 16-fold decrease in the cache's block size does not hurt temporal locality. 
Fig.~\ref{fig:4KB_locality} shows that increasing the block size even further, to 4KB, further decreases 
the cache's miss ratio. Unsurprisingly, the 4-fold increase in block size hurts the miss ratio for some workloads when using a small cache (<3\%). The cache size sweet spot slightly grows from 2\% to 3\%, which 
consistently provides a lower miss ratio than any cache size with 1KB blocks for all of the workloads. Our 
analysis clearly indicates that server workloads exhibit high spatial locality that can be captured even in 
modestly sized caches.


\noindent\textbf{Data region density.}
Our findings show that a DRAM cache in the 3\% range of the backing memory capacity range captures most of the locality of server applications. For that cache size, we further investigate the density of cache blocks as a metric for a given block size's efficiency (useful data vs. wasted data transfer), defining the density of a cache block as the fraction of 64B sub-blocks touched by the software during that block's residency in the cache. Fig.~\ref{fig:region_density} shows that all the workloads demonstrate high density of the memory traffic that gradually decreases with increasing the region size. While most workloads exhibit density over 70\% in the range of typical SCM row buffer sizes \dmitrii{(512-2048B)} \cite{suzuki:nonvolatile}, Web Serving and Data Analytics show density within 50-70\% due to lower data locality in read memory traffic that may cause wasteful read traffic. It is worth mentioning that the density of the writeback traffic is high (>70\%) for all the workloads that highlights high efficiency of bulk writeback operations that makes the case for amortization of conventionally slow SCM writes. 
\input{floats/float-sensitivity}

This analysis shows that the access patterns of server workloads demonstrate inherent spatial locality in 
memory traffic that allows the creation of large read and writeback requests to boost the effective SCM bandwidth, as analyzed in \S\ref{sec:latency_amortization}. At the same time, though, it indicates that the large transfer size may cause data overfetch.
\end{comment}

\begin{comment}
We first model a fully associative cache organized in 64B, hence any reuse captured is temporal. Fig.~\ref{fig:64B_locality} shows the miss ratio of such a cache as a function of the cache's capacity, which is expressed as a fraction of the dataset size; details on the methodology are provided in \S\ref{sec:method}. 

The workloads exhibit high diversity temporal locality: Data Analytics is insensitive to the cache
size, and exhibits very high temporal locality even for small caches. Web Search behavior demonstrates
a dramatic step function in miss ration when growing the cache from 3 to 6\%, indicating that its primary
working set is a small fraction of its dataset. Finally, the rest of the workloads exhibit a smoother
reduction in miss ratio as the cache size grows. In all cases, a cache in the reasonable 3-6\% capacity
range is capable of capturing a significant amount of the workloads' temporal locality, relaxing the
bandwidth demands from the backing memory by at least 50\%.\\

%\dmitrii{In comparison with overall temporal locality, writes locality of the workloads is significantly worse, and can be captured even by a cache with capacity in a range of 1-2\%, thus in average only 15-30\% of writes can be served by the cache~\ref{fig:wr_locality}. Hence, efficient cache design should focus on leveraging spatial locality to be efficient for the main with significant read/write disparity, like SCM.}

We use the same fully-associative cache methodology and increase the cache block size 
to study the spatial locality of the workloads as well. Fig.~\ref{fig:1KB_locality}~and~\ref{fig:4KB_locality} 
show the miss ratio for 1KB and 4KB blocks, respectively. 
\dmitrii{The change in miss ratio as compared to Fig.~\ref{fig:64B_locality}
captures the difference between the improvement from leveraging the workloads' spatial locality and 
the loss in temporal locality because of the 16- and 64-fold reduction in the number of distinct blocks in the cache.}
As most OSes use 4KB pages, we limit our spatial locality study
to block sizes up to 4KB.

Fig.~\ref{fig:1KB_locality} shows that organizing the cache of the same size in 1KB rather than 64B blocks
dramatically shrinks the miss ratio of all workloads to sub-5\% ranges even 
for modest caches sizes (>2\%). Furthermore, there is no perceivable benefit from growing the cache size beyond a 2\% capacity: the 16-fold decrease in
the cache's block size does not hurt temporal locality.

Fig.~\ref{fig:4KB_locality} shows that increasing the block size even further, to 4KB, further decreases the cache's miss ratio. Unsurprisingly, the 4-fold
increase in block size hurts the miss ratio for some workloads when using a small cache (<3\%). The cache size sweet spot slightly grows from 2\% to 3\%,
which consistently provides a lower miss ratio than any cache size with 1KB
blocks for all of the workloads. Our analysis clearly indicates that server workloads exhibit high spatial 
locality that can be captured even in modestly sized caches.
\\


\noindent\textbf{Data region density.}
Our findings show that a DRAM cache in the 3\% range of the backing memory capacity range captures most of the locality
of server applications. For that cache size, we further investigate the density of cache blocks as a metric for 
a given block size's efficiency (useful data vs. wasted data transfer), defining the density of a
cache block as the fraction of 64B sub-blocks touched by the software during that block's residency in the cache.
Motivated by SCM's read/write performance disparity, we study the density of clean and dirty blocks separately.

Fig.~\ref{fig:read_density} and \ref{fig:write_density} show the density for reads and writes, respectively.
The graphs clearly indicate that writebacks are significantly denser than reads. This characteristic is well-aligned
with the read/write disparity of SCM: it provides the opportunity to do large writebacks to improve SCM
bandwidth, as analyzed in \S\ref{sec:latency_amortization}. While the optimal block size
for reads is in the 512B-1KB range, for writes, even 4KB block are more than 50\% dense for all workloads.
This analysis shows that the access patterns of server workloads demonstrate inherent spatial locality in 
writes that allows the creation of large writebacks to boost the effective SCM bandwidth. At the same time, 
though, it indicates that the same large transfer size does not equally fit reads, which
account for the largest fraction of memory accesses, as it would result in data overfetch.

\end{comment}


\begin{comment}
\subsection{Summary}

Emerging SCM technologies are being investigated as replacements of DRAM as main memory. However, their increased access
latency and specifically the read/write disparity introduce a performance challenge for doing so.
A trend in modern servers that facilitates that integration is the recent introduction of DRAM caches, which are 
required to overcome the memory wall that arises from data-hungry server applications. 
The caches filter most of the traffic to the underlying memory, facilitating the replacement of DRAM with slower SCM.

Our first observation is that the limited bandwidth of SCM can be significantly boosted through bulk accesses.
Our second observation is that server applications exhibit high spatial locality in these caches. More interestingly,
writes are perceivably denser than reads, providing the opportunity to create larger write batches to amortize the higher
cost of SCM writes. Our two observations synergistically motivate a server memory hierarchy design that leverages the 
inherent spatial locality in server applications to facilitate SCM's integration, by improving its bandwidth.
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> obsolete/data_macros.tex <==
%define data values here

\begin{comment}
\newcommand{\perfVsCPUMax}{86$\times$}     
\newcommand{\perfVsPollockMax}{15$\times$}    
\newcommand{\energyVsCPUMax}{46$\times$}    
\newcommand{\energyVsPollockMax}{8$\times$}    
\newcommand{\efficiencyVsCPUMax}{46$\times$}    
\newcommand{\efficiencyVsPollockMax}{8$\times$}  

\newcommand{\perfCostVsPlanarDRAM}{3.8$\times$} 
\newcommand{\perfVsPlanarDRAM}{1.9$\times$}
\newcommand{\costVsPlanarDRAM}{1.4$\times$}
\newcommand{\perfCostVsBestDRAM}{2.3$\times$} 
\end{comment}

==> obsolete/design.tex <==
\section{Janus Memory Hierarchy}
\label{sec:design}

\begin{itemize}
    \item Design of a system that enables cache block size duality; virtual block size for writebacks. Mostly based on Virtual Write Queue.
    \item Focus on implications of original Virtual Write Queue work when applied to DRAM caches.
\end{itemize}

==> obsolete/float-density-csize.tex <==

\begin{figure}[t]
\centering
\subfloat[1KB regions.]{
       % \hspace{6pt}
        \includegraphics[width=1\columnwidth]{figures/density_vs_csize1KBreg}
        \label{fig:1KB_regions}}
\newline
\centering
\subfloat[8KB regions.] {
        \includegraphics[width=1\columnwidth]{figures/density_vs_csize8KBreg}
        \label{fig:8KB_regions}}
\caption{Region density of reads and writebacks for different region sizes. \alex{Need to decide what data to show and how to represent.}}
\label{fig:region_density}
%\vspace*{-9pt}
\end{figure}

==> obsolete/float-wr-locality.tex <==
\begin{figure}[t]
        \centering
        \includegraphics[width=\columnwidth]{figures/temp_loc_writes}
        \caption{Fraction of writes served by the cache.}
        \label{fig:wr_locality}
       % \vspace*{-9pt}
\end{figure}

